The GALAH Survey: Data Release 4

The stars of the Milky Way carry the chemical history of our Galaxy in their atmospheres as they journey through its vast expanse. Like barcodes, we can extract the chemical fingerprints of stars from high-resolution spectroscopy. The fourth data release (DR4) of the Galactic Archaeology with HERMES (GALAH) Survey, based on a decade of observations, provides the chemical abundances of up to 32 elements for 917 588 stars that also have exquisite astrometric data from the $Gaia$ satellite. For the first time, these elements include life-essential nitrogen to complement carbon, and oxygen as well as more measurements of rare-earth elements critical to modern-life electronics, offering unparalleled insights into the chemical composition of the Milky Way. For this release, we use neural networks to simultaneously fit stellar parameters and abundances across the whole wavelength range, leveraging synthetic grids computed with Spectroscopy Made Easy. These grids account for atomic line formation in non-local thermodynamic equilibrium for 14 elements. In a two-iteration process, we first fit stellar labels to all 1 085 520 spectra, then co-add repeated observations and refine these labels using astrometric data from $Gaia$ and 2MASS photometry, improving the accuracy and precision of stellar parameters and abundances. Our validation thoroughly assesses the reliability of spectroscopic measurements and highlights key caveats. GALAH DR4 represents yet another milestone in Galactic archaeology, combining detailed chemical compositions from multiple nucleosynthetic channels with kinematic information and age estimates. The resulting dataset, covering nearly a million stars, opens new avenues for understanding not only the chemical and dynamical history of the Milky Way, but also the broader questions of the origin of elements and the evolution of planets, stars, and galaxies.

==> tables/cannon_mask_percentage_1931.tex <==
\begin{table}[!ht]
    \centering
    \caption{Example of mask estimation for \textit{The Cannon} model creation. Listed are percentages of the spectrum that respond to an in-/decrease of each label above 0.001 and 0.0001 of the normalised flux.}
    \label{tab:cannon_mask_percentage}
    \begin{tabular}{cccc}
    \hline \hline
    Label &  Label change & $\vert \Delta f \vert > 0.001~/~\%$ & $\vert \Delta f \vert > 0.0001~/~\%$ \\
    \hline
    $T_\mathrm{eff}~/~\mathrm{K}$ & $\pm$250.0 & 85.1 & 99.2 \\
    $\log (g~/~\mathrm{cm\,s^{-2}})$ & $\pm$0.5 & 54.2 & 93.3 \\
    $\mathrm{[Fe/H]}$ & $\pm$0.25 & 95.6 & 99.6 \\
    $v_\mathrm{mic}~/~\mathrm{km\,s^{-1}}$ & $\pm$1.0 & 39.8 & 61.6 \\
    $\mathrm{[Li/Fe]}$ & $\pm$2.25 & 0.6 & 1.9 \\
    $\mathrm{[C/Fe]}$ & $\pm$1.0 & 95.1 & 99.2 \\
    $\mathrm{[N/Fe]}$ & $\pm$1.0 & 87.7 & 98.3 \\
    $\mathrm{[O/Fe]}$ & $\pm$2.0 & 82.9 & 98.6 \\
    $\mathrm{[Na/Fe]}$ & $\pm$1.0 & 30.1 & 74.0 \\
    $\mathrm{[Mg/Fe]}$ & $\pm$1.0 & 82.2 & 98.8 \\
    $\mathrm{[Al/Fe]}$ & $\pm$1.0 & 34.8 & 78.2 \\
    $\mathrm{[Si/Fe]}$ & $\pm$1.0 & 73.7 & 97.6 \\
    $\mathrm{[K/Fe]}$ & $\pm$1.0 & 2.1 & 29.1 \\
    $\mathrm{[Ca/Fe]}$ & $\pm$1.0 & 44.8 & 83.8 \\
    $\mathrm{[Sc/Fe]}$ & $\pm$1.0 & 4.8 & 10.6 \\
    $\mathrm{[Ti/Fe]}$ & $\pm$1.0 & 32.9 & 63.5 \\
    $\mathrm{[V/Fe]}$ & $\pm$1.0 & 18.8 & 35.5 \\
    $\mathrm{[Cr/Fe]}$ & $\pm$1.0 & 38.0 & 72.4 \\
    $\mathrm{[Mn/Fe]}$ & $\pm$1.0 & 13.7 & 48.0 \\
    $\mathrm{[Co/Fe]}$ & $\pm$1.0 & 19.9 & 39.7 \\
    $\mathrm{[Ni/Fe]}$ & $\pm$1.0 & 43.4 & 79.9 \\
    $\mathrm{[Cu/Fe]}$ & $\pm$1.0 & 0.8 & 2.7 \\
    $\mathrm{[Zn/Fe]}$ & $\pm$1.0 & 0.8 & 3.2 \\
    $\mathrm{[Rb/Fe]}$ & $\pm$1.0 & 0.1 & 0.3 \\
    $\mathrm{[Sr/Fe]}$ & $\pm$1.0 & 1.5 & 2.1 \\
    $\mathrm{[Y/Fe]}$ & $\pm$2.0 & 9.3 & 20.8 \\
    $\mathrm{[Zr/Fe]}$ & $\pm$1.0 & 3.3 & 8.5 \\
    $\mathrm{[Mo/Fe]}$ & $\pm$1.0 & 0.9 & 4.0 \\
    $\mathrm{[Ru/Fe]}$ & $\pm$1.0 & 1.0 & 3.2 \\
    $\mathrm{[Ba/Fe]}$ & $\pm$2.0 & 6.2 & 13.8 \\
    $\mathrm{[La/Fe]}$ & $\pm$1.0 & 3.3 & 4.5 \\
    $\mathrm{[Ce/Fe]}$ & $\pm$1.0 & 22.5 & 51.4 \\
    $\mathrm{[Nd/Fe]}$ & $\pm$1.0 & 10.3 & 16.5 \\
    $\mathrm{[Sm/Fe]}$ & $\pm$1.0 & 6.1 & 13.6 \\
    $\mathrm{[Eu/Fe]}$ & $\pm$1.0 & 0.3 & 0.5 \\
    \hline
    \end{tabular}
\end{table}


==> tables/vari_classifier_result.tex <==
\begin{table}
\centering
\caption{\textbf{Overlap of GALAH DR4 with \textit{Gaia} DR3 variability catalogues.} Classifications are taken from the \textit{gaiadr3.vari\_classifier\_result} table and described in \cite{Rimoldini2023}.}
\label{tab:overlap_gaiadr3_vari}
\begin{tabular}{ccc}
\hline \hline
Classification & DR4 allspec & DR4 allstar \\
\hline
ACV\vert CP\vert MCP\vert ROAM\vert ROAP\vert SXARI & 330 & 285 \\
ACYG & 45 & 34 \\
BCEP & 16 & 15 \\
BE\vert GCAS\vert SDOR\vert WR & 67 & 54 \\
CEP & 133 & 103 \\
CV & 3 & 3 \\
DSCT\vert GDOR\vert SXPHE & 16342 & 14477 \\
ECL & 4610 & 4074 \\
ELL & 95 & 11 \\
EP & 19 & 14 \\
LPV & 7351 & 6247 \\
RCB & 4 & 1 \\
RR & 561 & 401 \\
RS & 3950 & 3355 \\
S & 40 & 33 \\
SDB & 6 & 6 \\
SOLAR\_LIKE & 20027 & 17256 \\
SPB & 31 & 24 \\
SYST & 3 & 3 \\
WD & 1 & 1 \\
YSO & 1534 & 1096 \\
\hline
Total & 55168 & 47493 \\
\hline
\end{tabular}
\tablefootnote{Abbreviations: ACV ($\alpha$2 Canum Venaticorum), MCP and CP ((magnetic) chemically peculiar), ROAM and ROAP (rapidly oscillating Am- and Ap-type), SXARI (SXArietis), ACYG ($\alpha$ Cygni-type), BCEP ($\beta$ Cephei), BE (B-type emission line), GCAS ($\gamma$ Cassiopeiae), SDOR (SDoradus), WR (Wolf-Rayet), CEP (Cepheid, including anomalous Cepheid, BL Herculis variable, W Virginis variable, $\delta$ Cephei star, RV Tauri-type star, and generic type II Cepheids), CV (cataclysmic variable, excluding supernova and sym- biotic star), DSCT ($\delta$Scuti), GDOR ($\gamma$Doradus), SXPHE (SXPhoenicis), ECL (eclipsing binary including Algol type, $\beta$ Lyrae type, and W Ursae Majoris type), ELL (ellipsoidal variable), EP (star with exoplanet transits), LPV (long-period variable including long secondary period variable, Mira (oCeti) type, Mira or semi- regular  variable, OGLE small amplitude red giant, small amplitude red giant, and semi-regular variable of sub-types), RCB (R Coronae Borealis variable), RR (RR Lyrae star, including fundamental-mode, first overtone, double-mode and anomalous double-mode), RS (RS Canum Venaticorum variable), S (short-timescale object), SDB (subdwarf B star of type V1093 Herculis or V361 Hydrae), SOLAR\\_LIKE (solar-like, including BY Draconis type, rotating spotted star, and flaring stars), SPB (slowly pulsating B-type variable), SYST (symbiotic variable star, including Z Andromedae type), WD (variable white dwarf), YSO (young stellar object (YSO), including dipper stars, eruptive YSOs such as FU Orionis type variables, pulsating pre-main-sequence stars, Herbig Ae or Be types, including UX Orionis stars, and T Tauri stars).}
\end{table}

